Do the Benefits of Joint Models for Relation Extraction Extend to Document-level Tasks?

Two distinct approaches have been proposed for relational triple extraction - pipeline and joint. Joint models, which capture interactions across triples, are the more recent development, and have been shown to outperform pipeline models for sentence-level extraction tasks. Document-level extraction is a more challenging setting where interactions across triples can be long-range, and individual triples can also span across sentences. Joint models have not been applied for document-level tasks so far. In this paper, we benchmark state-of-the-art pipeline and joint extraction models on sentence-level as well as document-level datasets. Our experiments show that while joint models outperform pipeline models significantly for sentence-level extraction, their performance drops sharply below that of pipeline models for the document-level dataset.

==> dataset.tex <==
\section{Datasets Preparation}

For this study, we use a sentence-level dataset, NYT \cite{riedel2010modeling} and a document-level dataset, DocRED \cite{yao2019DocRED} for experiments. The context length of DocRED (avg. number of tokens around 197) is much longer than the NYT (avg. number of tokens around 37) dataset. We use the NYT dataset as it is for our experiments, but need to do some processing on DocRED to make it suitable for the joint models. Since the relation labels of the DocRED test set is not released, we use the original validation set as test set and split the training data for training and validation. We remove the documents with overlapping entity mentions in the training and validation set. We get 2,856 documents from the training set and 924 documents from the validation set. Then, we replace all entity mentions with the first occurring entity mention for each entity. This makes the task easier as models do not need to do co-reference resolution. The details of the dataset splits of the NYT and DocRED for our experiments are included in Table \ref{tab:data_stat}. In terms of size, NYT has large training data with shorter context length, whereas DocRED has significantly smaller training data with significantly longer context.


% The NYT dataset has 56,196 sentences in training data, and 5,000 sentences each in the validation data and test data. DocRED dataset has 3,053 documents in the training set and 1,000 documents each in the validation and test set. 

% We do some pre-processing on the DocRED to make it suitable for joint extraction models. 










==> experiments.tex <==
\section{Relation Extraction Approaches}

To compare the scalability of the relation extraction models, we perform experiments with 3 pipeline models and 5 joint models. 

\subsection{Pipeline Approaches}

Pipeline approaches solve the RE task in two steps. They use a NER model to identify the entities and then use a relation classification model to find the relations among them. Pipeline models take entities and entity mentions as input and predict a set of all possible relations from a pre-defined relation set. We use PL-Marker \cite{ye-etal-2022-packed} as the NER module and KD-DocRE \cite{tan-etal-2022-document}, SSAN \cite{Xu_Wang_Lyu_Zhu_Mao_2021}, and SAIS \cite{xiao-etal-2022-sais} as relation classification models for our experiments. We train PL-Marker on the NYT and DocRED datasets for corresponding experiments. For training and validation of the relation classification models, we use gold standard entity mentions. But during inference on the testset, we used the PL-Marker's generated entity mentions. 

\subsection{Joint Extraction Approaches}

Joint relation extraction models do not need a separate NER model. They identify the entities and relations in an end-to-end fashion. These models take the text (sentence or document) as input and output a set of relation tuples. This approach is difficult as two subtasks need to solved in a single model. We use 5 SOTA models for experiments. PtrNet \cite{nayak2019ptrnetdecoding} and REBEL \cite{huguet-cabot-navigli-2021-rebel-relation} are two models that use Seq2Seq approach for this task. PtrNet generates the index position of entities in text whereas REBEL generates the tokens for the tuples. OneRel \cite{Shang2022OneRelJE} uses a table-based tagging approach for this task. BiRTE \cite{Ren2022ASB} and GRTE \cite{Ren2021ANG} use a  tagging-based approach where they have a separate entity extraction process in their end-to-end modeling. We train these models on the NYT and DocRED datasets in an end-to-end fashion as described in the respective papers.






==> introduction.tex <==
\section{Introduction}

% Relation extraction is an important task in NLP for constructing or enriching knowledge bases (KB). With the advancement of deep learning models, research in this area also advanced rapidly in recent times. 

There are two distinct approaches for relation extraction: (i) Pipeline approach \cite{riedel2010modeling,zeng2014relation,zeng2015distant,nayak2019effective, jat2018attention} where entities are identified beforehand and models need to find the relations or no relation between two entities. (ii) Joint approach \cite{zeng2018copyre,hrlre2019takanobu,nayak2019ptrnetdecoding,Wei2020ANC,Wang2020TPLinkerSJ,Zheng2021PRGCPR,Li2021TDEERAE,Wei2020ANC,Yan2021APF,Shang2022OneRelJE} where models need to extract the possible entities and the relations among them. Most of the research focuses on sentence-level extraction, but recently document-level extraction gains popularity. 

Pipeline approaches consider only one entity pair at a time to find the relation. So they do not consider the interaction among the different entity pairs present in the same context. On the other hand, joint extraction approaches extract all relation tuples together, thus they are better suited to capture the interaction among the tuples. Experiments on the sentence-level dataset such as NYT \cite{riedel2010modeling} prove this point to an extent. But is this also true when we extend the task from sentence-level to document-level ? Are the sentence-level joint models scalable enough to apply directly to the document-level task ? NYT datasets contain only intra-sentence tuples where subject and object entities appear in the same sentence. But document-level datasets includes inter-sentence or cross-sentence tuples as well where the subject and object entity of a tuple appear in two different sentences of the document. How pipeline and joint models going to perform for intra-sentence vs inter-sentence tuples?  Most of the research in document-level extraction using dataset like DocRED \cite{yao2019DocRED} uses the pipeline approach and avoids the joint approach. In this work, we do a comparative study of the SOTA pipeline and joint models in the sentence-level and document-level relation extraction task and try to give insights regarding their performance and scalability for longer context.


